Event Extraction as Question Generation and Answering

Recent work on Event Extraction has reframed the task as Question Answering (QA), with promising results. The advantage of this approach is that it addresses the error propagation issue found in traditional token-based classification approaches by directly predicting event arguments without extracting candidates first. However, the questions are typically based on fixed templates and they rarely leverage contextual information such as relevant arguments. In addition, prior QA-based approaches have difficulty handling cases where there are multiple arguments for the same role. In this paper, we propose QGA-EE, which enables a Question Generation (QG) model to generate questions that incorporate rich contextual information instead of using fixed templates. We also propose dynamic templates to assist the training of QG model. Experiments show that QGA-EE outperforms all prior single-task-based models on the ACE05 English dataset.

==> 2.1_templates.tex <==
\subsection{Dynamic Template Design}
% Most publicly available event corpora such as ACE~\cite{doddington2004automatic} and Entities, Relations and Events (ERE)~\cite{song2015light} operate at the token or word level. To adapt the data to the QA framework, we need to first convert the token or word level annotations into question-answer pairs.
% In this section, we describe our method to automatically convert an event mention to a set of [ \texttt{argument role}, \texttt{role-oriented context-aware question}, \texttt{event arguments} ] pairs.
%\joel{it's not clear why one needs to do this conversion.  It feels like it comes out of nowhere}\di{added the motivation}

%\joel{what would help the models section is to have a paragraph in the beginning that outlines what happens in each subsection}
%\joel{I think an example is needed here, maybe this is where referring to Figure 2 can help} 
% The method is based on manually designed templates as prior work~\cite{du2020event}, but we create dynamic question templates which incorporate contextual information instead of using fixed templates. 
%\di{re-wrote the first paragraph}
% Given a sentence $s$, and an event trigger $e$ and a set of event arguments $\mathcal{A}$, $a_i = (r_i, w_i)$ for $a_i \in \mathcal{A}$, where $r_i$ is the role of the argument, and $w_i$ is the string of the argument, the simplest way is to use a simple template for each argument role.

% \noindent\fbox{
%  \parbox{\linewidth}{
% %  \begin{minipage}
%  \textbf{Sentence:} Even as the secretary of homeland security was putting his people on high alert last month, a 30-foot Cuban patrol boat with four heavily armed men landed on American shores, utterly undetected by the Coast Guard Secretary Ridge now leads.
 
%  \textbf{Event:} Movement.Transport
 
%  \textbf{Trigger:} landed
 
%  \textbf{Arguments:} boat (Vehicle-arg), men (Artifact-arg), shores (Destination-arg)
% }
%  }
\begin{table}[th]
    \centering
    \small
    \begin{tabular}{l}
    \hline
        % Template\\
         % \hline
        Who was the attacking agent? \\
        Who attacked [\texttt{Target}]?\\
        Who used [\texttt{Instrument}] in the attack?\\
        Who made the attack in [\texttt{Place}]?\\
        Who attacked [\texttt{Target}] using [\texttt{Instrument}]?\\
        Who attacked [\texttt{Target}] in [\texttt{Place}]?\\
        Who used [\texttt{Instrument}] in the attack in [\texttt{Place}]?\\
        Who attacked [\texttt{Target}] using [\texttt{Instrument}] in [\texttt{Place}]? \\ 
        \hline
    \end{tabular}
    \caption{Dynamic templates for \texttt{Attacker} role in \texttt{Conflict.Attack} event with different combinations of known argument roles based on ACE ontology.}
    \label{tab:templates}
\end{table}
% \subsubsection{Template Design for Dynamic Population}
Previous QA-based EE work~\cite{du2020event} designs simple templates and customizes them with only trigger information to generate the input questions to the QA model. 
However missing contextual information in the questions bottlenecks the performance of the QA model.
\joel{do we have any citations or examples to back this up?}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{fig/ace_example.pdf}
%     \caption{An ACE \texttt{Conflict.Attack} event with \textit{pummeled} as trigger word and three event arguments: \textit{coalition} (\texttt{Attacker}),  \textit{jets} (\texttt{Instrument}) and \textit{hills} (\texttt{Place}).}
%     \label{fig:ace_attacker}
% \end{figure}

In this work, we design dynamic templates for each role in the ACE ontology,\footnote{\url{https://www.ldc.upenn.edu/sites/www.ldc.upenn.edu/files/english-events-guidelines-v5.4.3.pdf}} to leverage different combinations of other argument roles into it.
% based on the ACE guidelines\footnote{https://www.ldc.upenn.edu/sites/www.ldc.upenn.edu/files/english-events-guidelines-v5.4.3.pdf}. 
For example, the \texttt{Conflict.Attack} event in ACE has four predefined argument roles: \texttt{Attacker}, \texttt{Target}, \texttt{Instrument} and \texttt{Place}\footnote{We follow the experimental setting of prior work, which excludes all the \texttt{Value} and \texttt{Timex}. Thus the argument roles such as \texttt{Time} are not included.}. 
For the \texttt{Attacker} role, we design eight templates using all of the possible combinations of the other roles included in the question (Table~\ref{tab:templates}). 
% The more argument roles that are pre-defined for a specific event type, the more templates we generate for each argument role associated with that event type. For example, for an event type with 2 predefined argument roles, we design two templates for each role. For an event type with five predefined argument roles, we have 16 templates for each role. 
%\joel{and this is all done via manually curated templates right?} \shihao{yes.}
Thus for the example in Figure~\ref{fig:ace_intro}, we obtain four questions for the \texttt{Attacker} role: (1)\textit{Who was the attacking agent?} (2) \textit{Who used jets in the attack?} (3) \textit{Who made the attack in hills?} (4) \textit{Who used jets in the attack in hills?}


% \begin{table*}[th]
%     \centering
%     \small
%     \begin{tabular}{c|c|c}
%     \hline
%         Target Role & Known Argument Roles&Template\\
%          \hline
%         \multirow{8}{*}{\texttt{Attacker}} & -&Who was the attacking agent? \\
%         {} & \texttt{Target} & Who attacked [\texttt{Target}]?\\
%         {} & \texttt{Instrument} & Who used [\texttt{Instrument}] in the attack?\\
%         {} & \texttt{Place} & Who made the attack in [\texttt{Place}]?\\
%         {} &  \texttt{Target}, \texttt{Instrument} & Who attacked [\texttt{Target}] using [\texttt{Instrument}]?\\
%         {} &  \texttt{Target}, \texttt{Place}&Who attacked [\texttt{Target}] in [\texttt{Place}]?\\
%         {} &  \texttt{Instrument}, \texttt{Place} & Who used [\texttt{Instrument}] in the attack in [\texttt{Place}]?\\
%         {} &   \texttt{Target}, \texttt{Instrument}, \texttt{Place} & Who attacked [\texttt{Target}] using [\texttt{Instrument}] in [\texttt{Place}]? \\ 
%         \hline
%     \end{tabular}
%     \caption{Templates for argument role \texttt{Attacker} in \texttt{Conflict.Attack} event with different combinations of known argument roles.}
%     \label{tab:templates}
% \end{table*}


% \begin{itemize}
%     \item \textbf{Without any argument known:} Who was the attacking agent?
%     \item \textbf{Know \texttt{Target}: } Who attacked [\texttt{Target}]?
%     \item \textbf{Know \texttt{Instrument}: } Who used [INSTRUMENT-ARG] in the attack?
%     \item \textbf{Know \texttt{Place}: } Who made the attack in [PLACE-ARG]?
%     \item \textbf{Know \texttt{Target} and \texttt{Instrument}: } Who attacked [TARGET-ARG] using [INSTRUMENT-ARG]?
%     \item \textbf{Know \texttt{Target} and \texttt{Place}: } Who attacked [TARGET-ARG] in [PLACE-ARG]?
%     \item \textbf{Know \texttt{Instrument} and \texttt{Place}: } Who used [INSTRUMENT-ARG] in the attack in [PLACE-ARG]?
%     \item \textbf{Know \texttt{Target}, \texttt{Instrument} and \texttt{Place}: } Who attacked [TARGET-ARG] using [INSTRUMENT-ARG] in [PLACE-ARG]?
% \end{itemize}




% \noindent\textbf{Template Filling} By using the dynamic templates, we can pick up different templates based on the combination of contextual arguments, and fill in corresponding arguments to generate multiple questions.
% When we convert the event mention into [ \texttt{argument role}, \texttt{role-oriented context-aware question}, \texttt{event arguments} ] pairs for a specific argument role, we first retrieve all of the templates associated with the role. 
% For example, we can generate four questions for the \texttt{Attacker} role in the \textit{Attack} event in Figure~\ref{fig:ace_attacker}: (1)\textit{Who was the attacking agent?}(2) \textit{Who used jets in the attack?} (3) \textit{Who made the attack in hills?} (4) \textit{Who used jets in the attack in hills?}
% , based on the templates (1) \textit{Who was the attacking agent?} (2) \textit{Who used [\texttt{Instrument}] in the attack?} (3) \textit{Who made the attack in [\texttt{Place}]?} (4) \textit{Who used [\texttt{Instrument}] in the attack in [\texttt{Place}]?}

% in Figure~\ref{fig:ace_attacker}, we have a sentence `\textit{That's because coalition fighter jets pummeled this Iraqi position on the hills above Chamchamal and Iraqi troops made a hasty retreat.}' and a \texttt{Conflict.Attack} event mention with \textit{pummeled} as the trigger word and \textit{coalition},  \textit{jets} and \textit{hills} as three event arguments with roles of \texttt{Attacker}, \texttt{Instrument} and \texttt{Place} respectively. To generate the questions for the \texttt{Attacker} role in this sentence, we first retrieve all of the eight templates designed for it (Table~\ref{tab:templates}). Then we filter out the templates that contain the argument roles not mentioned in the sentence. In this example, \texttt{Target} is not mentioned, so we exclude all the templates with [\texttt{Target}] slot. We then have four templates as follows:
% \begin{itemize}
%     \item Who was the attacking agent?
%     \item Who used [\texttt{Instrument}] in the attack?
%     \item Who made the attack in [\texttt{Place}]?
%     \item Who used [\texttt{Instrument}] in the attack in [\texttt{Place}]?
% \end{itemize}

% Lastly, we fill in the slots with corresponding event arguments, and obtain the final questions for the \texttt{Attacker} argument role:
% \joel{I can understand how it would be easy to fill in the slots given the gold standard - is that how it is done in training?  How is it done inference? }\di{that's why we propose the QG model, it is trained to generate the most context-aware questions based on raw sentence and target argument role only}
% \begin{itemize}
%     \item Who was the attacking agent?
%     \item Who used jets in the attack?
%     \item Who made the attack in hills?
%     \item Who used jets in the attack in hills?
% \end{itemize}

% If there are multiple arguments associated with the role slot, we randomly pick up one to form the questions. By applying the steps described in \textbf{Template Design} and \textbf{Template Filling}, not only do we generate questions that incorporate more information from context, but we also augment the training data significantly (from 4,859 to 15,426 for our training set).%\joel{do we have a sense of how many more questions we generate?}\di{added the numbers} 
% The question for one argument role can be `decomposed' into multiple ones as long as there are more than two argument roles mentioned in the event context.
% Because we convert one event mention for event argument into multiple ones as long as there are more than two argument roles in the event mention.
% We generate more context-aware questions by incorporating information from other arguments by apply the steps described above. 
% Moreover, we also augment the training data. Because we can convert one annotation for event argument into multiple ones as long as there are more than two argument roles in the event mention.
% Procedure to generate context-aware question-answer pairs for ACE dataset.

% \begin{equation}
%     query_{template} = f_{template}(s_i, A_i, a_i)
% \end{equation}



==> 7_Ethics.tex <==
\section*{Ethics Statement}

